Two-sample testing of high-dimensional linear regression coefficients via complementary sketching

We introduce a new method for two-sample testing of high-dimensional linear regression coefficients without assuming that those coefficients are individually estimable. The procedure works by first projecting the matrices of covariates and response vectors along directions that are complementary in sign in a subset of the coordinates, a process which we call 'complementary sketching'. The resulting projected covariates and responses are aggregated to form two test statistics, which are shown to have essentially optimal asymptotic power under a Gaussian design when the difference between the two regression coefficients is sparse and dense respectively. Simulations confirm that our methods perform well in a broad class of settings and an application to a large single-cell RNA sequencing dataset demonstrates its utility in the real world.

==> contents/acknowledgement.tex <==
%!TEX root = ../compsket.tex

\textbf{Acknowledgements.} This work was primarily supported by the Royal Society grant IEC/NSFC/170119. In addition, the research of FG was supported by NSFC grants 11701095 and 11690013 and that of TW was supported by EPSRC grant EP/T02772X/1. We would like to thank Chenqu Suo for suggesting the dataset and offering her valuable insights in the real data analysis. We thank the anonymous reviewers for helpful and constructive comments on an earlier draft.


==> contents/additional.tex <==
%!TEX root = ../compsket_supp.tex

\section{Proofs of the rest of theoretic results}
\label{Sec:Additional}
We collect here proofs of the remaining theoretical results omitted in the main text.

To prove Proposition~\ref{Prop:WtW-general}, we need the following proposition, which considers tail bounds for $\|Wu\|$ for a fixed $u\in\mathcal{S}^{p-1}$ in the special case $\Sigma = I_p$.
\begin{prop}
    \label{Prop:WtW}
    Under the conditions of Proposition~\ref{Prop:WtW-general}, we further assume $\Sigma=I_p$. There exists a random sequence $(h_n)_n$ such that $h_n \xrightarrow{\mathrm{a.s.}} 4\kappa_1$ for $\kappa_1$ defined in Lemma~\ref{lemma:spectral-limit} and that for any sequence $(\delta_n)_n$ satisfying $\log(1/\delta_n) = \smallO(p)$, we have for all large $p$ that
    \[
    \mathbb{P}\biggl\{\biggl| \frac{1}{n} (W^\top W)_{1,1} - h_n\biggr| \!>\! (8+\smallO(1)) \sqrt\frac{\log (1/\delta_n)}{n} \bigl( (\kappa_1 + \kappa_2) \sqrt{n/p} + \kappa_1 \bigr)\biggr\}\!\leq\! \delta_n.
    \]
\end{prop}
\begin{proof}
Let $X = QT$ be the QR decomposition of $X$, which is almost surely unique if we require the upper-triangular matrix $T$ to have non-negative entries on the diagonal.

Let $Q_1$ be the submatrix obtained from the first $n_1$ rows of $Q$. From Lemma~\ref{Lemma:GaussianQR}, $Q_1$ and $T$ are independent and $T$ has independent entries distributed as $T_{j,j} = t_j > 0$ with $t_j^2\sim \chi^2_{n-j+1}$ for $j\in[p]$ and $T_{j,k} = z_{j,k} \sim N(0,1)$ for $1\leq j < k\leq p$.

Define $B := Q_1^\top Q_1$ and let $B = V\Lambda V^\top$ be its eigendecomposition, which is almost surely unique if we require the diagonal entries of $\Lambda$ to be non-increasing and the diagonal entries of $V$ to be nonnegative. By Lemma~\ref{Lemma:GaussianQR}, $Q$ is uniformly distributed on $\mathbb{O}^{n\times p}$, which means $Q \stackrel{\mathrm{d}}{=} QH$ for any $H\in\mathbb{O}^{p\times p}$.
Consequently, $Q_1 \stackrel{\mathrm{d}}{=} Q_1 H$ and $B\stackrel{\mathrm{d}}{=} H^\top B H = (H^\top V) \Lambda (H^\top V)^\top$. Since the group $\mathbb{O}^{p\times p}$ acts transitively on itself through left multiplication, the joint density of $V$ and $\Lambda$ must be a function of $\Lambda$ only. In particular, $V$ and $\Lambda$ are independent.

Note that $X_1 = Q_1 T$. Thus, $X_1^\top X_1 = T^\top B T$ and $X_2^\top X_2 = T^\top (I_p-B)T$. By Lemma~\ref{Lemma:GramW}, we have
\begin{align}
W^\top W &= 4 X_1^\top A_1 A_1^\top X_1 = 4 (X_1^\top X_1)(X_1^\top X_1 + X_2^\top X_2)^{-1}(X_2^\top X_2)\nonumber\\
& = 4 T^\top B(I_p - B) T = 4 T^\top V \Lambda(I_p-\Lambda) V^\top T.\label{Eq:WtW}
\end{align}
Let $1\geq \lambda_1\geq \cdots\geq \lambda_p\geq 0$ be the diagonal entries of $\Lambda$. Define $a_j = \lambda_j(1-\lambda_j)$ for $j\in[p]$ and set $a := (a_1,\ldots,a_p)$. We can write $t_1^2 = s_1^2 + r_1^2$ with $s_1^2\sim \chi^2_p$ and $r_1^2\sim\chi^2_{n-p}$ such that $s_1\geq 0$, $r_1\geq 0$ are independent of each other and independent of everything else. By Lemma~\ref{Lemma:GaussianQR}, we have that $G_{j,1}:=s_1 V_{j,1}$ for $j\in[p]$ are independent $N(0,1)$ random variables. Note that
\[
\frac{1}{4}(W^\top W)_{1,1} = \sum_{j=1}^p t_1^2 a_j V_{j,1}^2 = \frac{t_{1}^2}{s_{1}^2} \sum_{j=1}^p a_j G_{j,1}^2.
\]
Let $\delta = \delta_n>0$ be chosen later. By \citet[Lemma~1]{LaurentMassart2000}, applied conditionally on $a$, we have with probability at least $1-6\delta$ that all the following inequalities hold:
\begin{gather*}
\|a\|_1 - 2\|a\|_2\sqrt{\log\frac{1}{\delta}}\leq \sum_{j=1}^p a_j G_{j,1}^2 \leq \|a\|_1 + 2\|a\|_2\sqrt{\log\frac{1}{\delta}} + 2\|a\|_\infty \log\frac{1}{\delta},\\
p-2\sqrt{p \log\frac{1}{\delta}}\leq s_1^2 \leq p+2\sqrt{p\log\frac{1}{\delta}}+2\log\frac{1}{\delta},\\
n-2\sqrt{n\log\frac{1}{\delta}}\leq t_1^2 \leq n+2\sqrt{n\log\frac{1}{\delta}}+2\log\frac{1}{\delta}.
\end{gather*}
Keeping in mind that $\|a\|_\infty\leq 1/4$, we have with probability at least $1-6\delta$ that
\begin{align*}
&\frac{n-2\sqrt{n\log(1/\delta)}}{p+2\sqrt{p\log(1/\delta)}+2\log(1/\delta)}\bigl\{\|a\|_1 - 2\|a\|_2\sqrt{\log(1/\delta)}\bigr\}  \leq
\frac{1}{4}(W^\top W)_{1,1} \\
&\quad \leq \frac{n+2\sqrt{n\log (1/\delta)}+2\log(1/\delta)}{p-2\sqrt{p\log (1/\delta)}}\bigl\{\|a\|_1 + 2\|a\|_2\sqrt{\log(1/\delta)} + \frac{1}{2}\log(1/\delta)\bigr\}
\end{align*}
If $\log(1/\delta) = \smallO(p)$, then for each $p$ with probability at least $1-6\delta$, we have that
\begin{equation}
    \begin{aligned}
      \biggl| \frac{(W^\top W)_{1,1}}{4} & - \frac{n}{p} \| a \|_1 \biggr|   \leq \| a \|_1 \frac{2 \sqrt{n \log(1 / \delta)}}{ p} \bigl( 1 + \!\sqrt{n/p}\bigr) \\
     & + \frac{n}{p} \biggl\{2 \| a \|_2 \sqrt{\log(1/ \delta)} + \frac{\log(1/\delta)}{2} \biggr\} \\
     & + \mathcal{O}_s\biggl(\frac{\|a\|_1\log(1/\delta)}{p}+\frac{\|a\|_2\log(1/\delta)}{\sqrt{p}}+\frac{\log^{3/2} (1/\delta)}{p^{1/2}}\biggr).
    \end{aligned}
     \label{Eq:ErrorTerms}
\end{equation}
By the definition of $B$, we have for $H:=T(X^\top X)^{-1/2}\in\mathbb{O}^{p\times p}$ that
\[
H^\top B H = H^\top T^{-\top}X_1^\top X_1 T^{-1}H = (X^\top X)^{-1/2} (X_1^\top X_1)(X^\top X)^{-1/2},
\]
which follows the matrix-variate Beta distribution $\mathrm{Beta}_p(n_1/2, n_2/2)$ as defined before Lemma~\ref{lemma:spectral-limit}. Hence, the diagonal elements of $\Lambda$ are the same as the eigenvalues of a $\mathrm{Beta}_p(n_1/2, n_2/2)$ random matrix. By~\eqref{Eq:ErrorTerms}, for each $p$, with probability at least $1-6\delta$, we have
\begin{equation}
    \label{Eq:OneVectorTail}
    \begin{aligned}
        \biggl|  (W^\top W)_{1,1}  -\frac{4n}{p}\|a\|_1\biggr| & \leq 8 \sqrt{n \log (1/\delta)} \bigl( (\kappa_1 + \kappa_2) \sqrt{n/p} + \kappa_1 \bigr) \\
        & \qquad \qquad \quad + \mathcal{O}_s\biggl(\log(1/\delta) + \frac{\log^{3/2}(1/\delta)}{p^{1/2}}\biggr).
    \end{aligned}
\end{equation}
The desired result follows by taking $h_n = 4\|a\|_1/p$ and observing that by Lemma~\ref{lemma:spectral-limit} $h_n \to 4\kappa_1$ almost surely.
\end{proof}

With Proposition~\ref{Prop:WtW}, we are now in a position to prove Proposition~\ref{Prop:WtW-general} in its general form.

\begin{proof}[Proof of Proposition~\ref{Prop:WtW-general}]
Let $V_i := X_i \Sigma^{-1/2}, i = 1, 2$ and set $V = (V_1^\top, V_2^\top)^\top$. Then each row of $V$ follows $N(0, I_p)$ and is independent of each other. We have
\begin{align*}
    W^\top W & = 4 (X_1^\top X_1) (X^\top X)^{-1} (X_2^\top X_2) \\
    & = 4 (\Sigma^{1/2} V_1^\top V_1 \Sigma^{1/2}) (\Sigma^{-1/2} (V^\top V)^{-1} \Sigma^{-1/2}) (\Sigma^{1/2} V_2^\top V_2 \Sigma^{1/2}) \\
    & =  4\Sigma^{1/2} V_1^\top V_1 (V^\top V)^{-1} V_2^\top V_2 \Sigma^{1/2} \stackrel{\mathrm{d}}{=} \Sigma^{1/2} (W_I^\top W_I) \Sigma^{1/2},
\end{align*}
where $W_I$ is the complementarily sketched design matrix when all entries of $X$ are independent standard normals (i.e.\ $\Sigma = I_p$). Let $h_n$ be the random sequence satisfying Proposition~\ref{Prop:WtW} and define $\Delta := W^\top W/ n - h_n  \Sigma$ and $\Delta_I := W_I^\top W_I / n - h_n I_p$. We start by controlling the $\ell$-sparse operator norm of $\Delta$ for an arbitrary $\ell\in[p]$. By Lemma~\ref{Lemma:Net}, there exists a $1/4$-net $\mathcal{N}_\ell$ of $\{v\in\mathcal{S}^{p-1}: \|v\|_0\leq \ell\}$ of cardinality at most $\binom{p}{\ell}9^\ell$, such that
\begin{align}
\label{Eq:Prop2tmp1}
\|\Delta\|_{\ell,\mathrm{op}} &= 2\sup_{u\in \mathcal{N}_\ell} u^\top \Delta u \stackrel{\mathrm{d}}{=} 2\sup_{u\in \mathcal{N}_\ell} (\Sigma^{1/2}u)^\top \Delta_I (\Sigma^{1/2}u) \nonumber\\
&\leq 2\|\Sigma \|_{k,\mathrm{op}} \sup_{u\in\mathcal{N}_\ell'} u^\top \Delta_I u \leq 2\overline{\lambda}\sup_{u\in\mathcal{N}_\ell'} u^\top \Delta_I u,
\end{align}
where $\mathcal{N}_\ell' := \{\Sigma^{1/2}u / \|\Sigma^{1/2}u\|_2: u\in\mathcal{N}_\ell\}$. We claim that for any $u\in\mathcal{S}^{p-1}$, we have $u^\top \Delta_I u \stackrel{\mathrm{d}}= e_1^\top \Delta_I e_1$. This is because for any $H\in\mathbb{O}^{p\times p}$, we have $V\stackrel{\mathrm{d}}= VH$ and hence by Lemma~\ref{Lemma:GramW} that
\begin{align}
H^\top W_I^\top W_I H &= 4(H^\top V_1^\top V_1H)(H^\top V^\top VH)^{-1}(H^\top V_2^\top V_2H)\nonumber\\ &\stackrel{\mathrm{d}}
=4(V_1^\top V_1)(V^\top V)^{-1}(V_2^\top V_2)= W_I^\top W_I,\label{Eq:RotationalSymmetry}
\end{align}
which in particular implies our claim.  Consequently, by Proposition~\ref{Prop:WtW} and a union bound, when $\log(1/\delta) = \smallO(p)$, we have with probability at least $1- 6|\mathcal{N}_\ell|\delta$ that
\begin{equation}
\label{Eq:Prop2tmp3}
    \| \Delta\|_{\ell,\mathrm{op}} \leq (16+\smallO(1))\overline{\lambda}\sqrt\frac{\log(1/\delta)}{n}\bigl\{(\kappa_1+\kappa_2)\sqrt{n/p}+\kappa_1\bigr\}.
\end{equation}

To prove~\eqref{Eq:WtWdiag-1}, we recall $\diag(\Sigma) = I_p$ and set $\ell=1$ and $\delta=p^{-3}$ in~\eqref{Eq:Prop2tmp3} to obtain with probability at least $1-54p^{-2}$ that
\begin{equation}
    \begin{aligned}
        \max_{j\in[p]}\biggl|\frac{(W^\top W)_{j,j}}{nh_n} & - 1\biggr|  = \frac{1}{h_n}\|\Delta\|_{1,\mathrm{op}} \\
        & \leq \frac{(16+\smallO(1))\overline{\lambda}}{h_n}\sqrt\frac{3\log p}{n}\bigl\{(\kappa_1+\kappa_2)\sqrt{n/p}+\kappa_1\bigr\}.
    \end{aligned}
\label{Eq:Prop2tmp4}
\end{equation}
The first conclusion follows by noting that $h_n\to 4\kappa_1$ and an application of the Borel--Cantelli lemma (since $p^{-2}$ is summable).

To prove~\eqref{Eq:kopNorm-1}, we set $\ell=k$ and $\delta = (10ep/k)^{-(k+4)}$. By~\eqref{Eq:klogpovern-1}, we have $\log(1/\delta) = (k+4)\log(10ep/k) = \smallO(p)$ and
\begin{align*}
|\mathcal{N}|\delta & \leq 9^k\binom{p}{k}\biggl(\frac{10ep}{k}\biggr)^{-(k+4)}  \leq \biggl(\frac{9ep}{k}\biggr)^k\biggl(\frac{10ep}{k}\biggr)^{-(k+4)} \\
& \leq \frac{0.9^k}{(ep/k)^4} \leq \max(p^{-2}, 0.9^{\sqrt{p}}).
\end{align*}
By the Borel--Cantelli lemma,
\begin{equation}
\label{Eq:Prop2tmp2}
    \| \Delta\|_{k,\mathrm{op}} \leq (16+\smallO(1))\overline{\lambda}\sqrt\frac{(k+4)\log(10ep/k)}{n}\bigl\{(\kappa_1+\kappa_2)\sqrt{n/p}+\kappa_1\bigr\}.
\end{equation}
holds for all but finitely many $p$.  We work on $p$ sufficiently large such that \eqref{Eq:Prop2tmp2} holds henceforth. Define $\hat D:=\diag(W^\top W) / (n h_n)$. By \eqref{Eq:Prop2tmp4} and a Taylor expansion, we have that $\|\hat D^{-1/2} - I\|_{\mathrm{op}} = (1 +\smallO(1))(2h_n)^{-1}\|\Delta\|_{1,\mathrm{op}}$. Thus,
\begin{align*}
\|\hat D^{-1/2} W^\top & W \hat D^{-1/2} -  W^\top W  \|_{k,\mathrm{op}} \\
& \leq \|\hat D^{-1/2} - I\|_{\mathrm{op}}\| W^\top W \|_{k,\mathrm{op}} (1+\|\hat D^{-1/2}\|_{\mathrm{op}})\\
&\leq (2+\smallO(1))\frac{\|\Delta\|_{1,\mathrm{op}}}{2h_n} \|n\Delta+nh_n\Sigma\|_{k,\mathrm{op}}
\leq (1+\smallO(1)){n\overline{\lambda}\|\Delta\|_{1,\mathrm{op}}}%{2}.
\end{align*}
where the final bound follows from~\eqref{Eq:Prop2tmp2} and the fact that $\|\Sigma\|_{k,\mathrm{op}}\leq \overline{\lambda}$. Consequently, noting $h_n\to 4\kappa_1$, for all large $p$ we have
\begin{align*}
\|\tilde W^\top \tilde W - \Sigma\|_{k,\mathrm{op}} &= \frac{1}{h_n} \|\hat D^{-1/2} W^\top W \hat D^{-1/2}/n - h_n \Sigma\|_{k,\mathrm{op}} \\
&\leq \frac{1}{h_n}\|\Delta\|_{k,\mathrm{op}} + \frac{1}{nh_n}\|\hat D^{-1/2} W^\top W \hat D^{-1/2} -  W^\top W  \|_{k,\mathrm{op}} \\
&\leq \frac{1}{h_n} (\|\Delta\|_{k,\mathrm{op}} + \overline{\lambda} \|\Delta\|_{1,\mathrm{op}}) \\
& \leq C_{s,r}\biggl\{\overline{\lambda}\sqrt\frac{k\log(ep/k)}{n}+\overline{\lambda}^2\sqrt\frac{\log p}{n}\biggr\},
\end{align*}
for $C_{s,r} := 9 (1+\sqrt{1+1/s}+\sqrt{s+r-1+1/s+1/r})$, which completes the proof.
\end{proof}


\begin{proof}[Proof of Corollary~\ref{Cor:SparseUpper}]
The first inequality follows from the definition of~$\mathcal{M}_X(k,\rho)$. An inspection of the proofs of Theorems~\ref{Thm:Null} and~\ref{Thm:Alternative} of the main text reveals that both results only depend on the complementary-sketched model $Z=W\theta+\xi$, and hence hold uniformly over $(\beta_1,\beta_2)$. Thus, we have from Theorem~\ref{Thm:Null} that $\sup_{\beta\in\mathbb{R}^p} P_{\beta,\beta}^X (\psi^{\mathrm{sparse}}_{\lambda,\tau}\neq 0) \xrightarrow{\mathrm{a.s.}} 0$ and from Theorem~\ref{Thm:Alternative} that $\sup_{\beta_1,\beta_2\in\mathbb{R}^p: (\beta_1-\beta_2)/2\in\Theta_{p,k}(\rho)} P_{\beta,\beta}^X (\psi^{\mathrm{sparse}}_{\lambda,\tau}\neq 1) \xrightarrow{\mathrm{a.s.}} 0$. Combining the two completes the proof.
\end{proof}


\begin{proof}[Proof of Theorem~\ref{Thm:AlternativeDense}]
%\fn{Here we prove a slight stronger version of Theorem~\ref{Thm:AlternativeDense}, where $\eta :=\hat\sigma^2 ( m + 2 \sqrt{m(1+\varepsilon)\log p} + 2 (1 + \varepsilon) \log p) $ for any $0 < \varepsilon < 5$.}
As in the proof of Theorem~\ref{Thm:Alternative}, we work with a deterministic sequence of $W$ such that~\eqref{Eq:WtWdiag-1} and \eqref{Eq:kopNorm-1} are satisfied.
Furthermore, by Condition~\ref{cond:sigma-strong}, we henceforth work on the almost sure event $\Omega_\sigma = \{ |\hat\sigma/\sigma - 1 | = \smallO(p^{-1/2}\log^{1/2} p) \}$.
For $\tilde\theta = (\tilde\theta_1,\ldots,\tilde\theta_p)^\top$ such that $\tilde\theta_j := \theta_j \|W_j\|_2$, we have from~\eqref{Eq:ZW} that
\(
Z = \tilde W \tilde\theta + \xi,
\)
for $\xi \sim N_m(0, \sigma^2 I_m)$. Hence, under the null hypothesis,  $(\|Z\|_2^2/\sigma^2) \sim \chi^2_m$, which by \citet[Lemma~1]{LaurentMassart2000} yields that
\[
    \mathbb{P}\bigl\{\|Z\|_2^2 / \sigma^2 \geq m + 2\sqrt{m\log(1/\delta)} + 2\log(1/\delta) \bigr\} \leq \delta.
\]
%Setting $\delta=p^{-2}$, for $\eta=\hat{\sigma} (m +2^{3/2}\sqrt{m\log p}+4\log p)$, we have by the Borel--Cantelli lemma that $\psi^{\mathrm{dense}}_\eta(X_1,X_2,Y_1,Y_2) \xrightarrow{\mathrm{a.s.}} 0$.
We set $\delta = p^{- (1+\varepsilon/2)}$ and have for $\eta_0=\sigma^2 (m +2\sqrt{(1+\varepsilon/2)m\log p}+2(1+\varepsilon/2)\log p)$, $\eta = \hat\sigma^2 ( m + 2 \sqrt{m(1+\varepsilon)\log p} + 2 (1 + \varepsilon) \log p)  \ge \eta_0$ on $\Omega_\sigma$ for all $p$ sufficiently large.
We bound, for all $p$ sufficiently large,
\begin{equation*}
    \mathbb{P} ( \| Z \|^2 \ge \eta) \le \mathbb{P}( \|Z\|^2 \ge \eta_0) \le p^{-(1+\varepsilon/2)},
\end{equation*}
whence, by the Borel--Cantelli lemma, we have $\psi^{\mathrm{dense}}_\eta(X_1,X_2,Y_1,Y_2) \xrightarrow{\mathrm{a.s.}} 0$.


On the other hand, under the alternative, $(\|Z\|_2^2/\sigma^2) \sim \chi^2_m(\|W\theta\|_2^2)$. Observe from~\eqref{Eq:WtWdiag-1} and~\eqref{Eq:kopNorm-1} that
\begin{align*}
        \|W\theta\|_2^2&=\|\tilde W\tilde \theta\|_2^2 = \|\Sigma^{1/2}\tilde\theta\|_2^2 + \tilde\theta^\top (\tilde W^\top \tilde W - \Sigma)\tilde\theta \\
        &\geq  \|\tilde\theta\|_2^2\bigl(\underline{\lambda}-\|\tilde W^\top \tilde W - \Sigma\|_{k,\mathrm{op}}\bigr)\\
&\geq (4\underline{\lambda}-\smallO(1))n\kappa_1\rho^2 \geq (8-\smallO(1))\sigma^2 \sqrt{m\log p}.
\end{align*}
By a similar argument, we also have $\|W\theta\|_2^2 \leq (4\overline{\lambda}+\smallO(1))n\kappa_1\rho^2 = \smallO(m)$.
Thus, by \citet[Lemma~8.1]{Birge2001}, we have with probability at least $1-p^{-2}$ that
\begin{align*}
\|Z\|_2^2/\sigma^2 &\geq  m + \|W\theta\|_2^2 - 2\sqrt{(2m+4\|W\theta\|_2^2)\log p}\\
&\geq m + (8-2\sqrt{2}-\smallO(1))\sqrt{m\log p}
\end{align*}
%which is at least $\eta = \hat\sigma^2 ( m+\sqrt{8 m\log p}+4\log p)$ for all sufficiently large $p$. 
which is at least $\eta = \hat\sigma^2 ( m + 2\sqrt{2(1+\varepsilon)m\log p} + 2(1+\varepsilon) \log p) \le $ for all $p$ sufficiently large and any $\varepsilon\in (0, 5]$, conditionally on the almost sure event~$\Omega_\sigma$. 

Consequently, we have $\mathbb{P}(\|Z\|_2^2\leq \eta)\leq p^{-2}$ for all large $p$. As $p^{-2}$ is summable, by the Borel--Cantelli lemma,  $\psi^{\mathrm{dense}}_\eta(X_1,X_2,Y_1,Y_2)\xrightarrow{\mathrm{a.s.}}1$.
%\fn{Take $\varepsilon=1$ in the preceding arguments gives the theorem statement where $\eta = \hat\sigma^2( m + 2\sqrt{2m\log p} + 4 \log p)$.}
\end{proof}

\begin{proof}[Proof of Theorem~\ref{Thm:LowerBoundDense}]
Note that since $k\leq p^{\alpha}$ for $\alpha<1$, condition~\eqref{Eq:klogpovern-1} is satisfied and hence we can work with a deterministic sequence of $W$ satisfying~\eqref{Eq:WtWdiag-1} and~\eqref{Eq:kopNorm-1}. Similar to the proof of Theorem~\ref{Thm:LowerBound}, we write $\Sigma = \Sigma_0 + \Gamma$ for some $\Sigma_0\in\mathrm{RowSp}(D)$ with $\|\Sigma_0\|_{\max}\leq 1$ and $\|\Gamma\|_{\max}=\smallO(D/(k\log p))$. We follow the proof of Theorem~\ref{Thm:LowerBound} up to~\eqref{Eq:FactorI_tbc}. 

Now, since $\rho^2 = \smallO(p^{-1/2}\min\{\log^{-1/2} (ep/k), D^{-3/2}\})$, we have by~\eqref{Eq:rhotovartheta} that  $\mathbb{E}(e^{2\tilde\theta^\top (\tilde W^\top \tilde W - \Sigma_0)\tilde\theta'}) = 1+\smallO(1)$. It remains to show that  $\mathbb{E}(e^{2\tilde\theta^\top  \Sigma_0\tilde\theta'}) = 1+\smallO(1)$. To this end, we have by Lemma~\ref{Lemma:Chaos2} that
\begin{align*}
\mathbb{E}(e^{2\tilde\theta^\top \Sigma_0\tilde\theta'}) &\leq  \biggl\{1 + \frac{Dk}{p}\bigl(\cosh(2\vartheta^2 D) - 1\bigr)\biggr\}^k \leq \biggl\{1 + \frac{Dk}{p} \bigl(2+\smallO(1)\bigr)\vartheta^4 D^2\biggr\}^k\\
& \leq \exp\biggl\{\frac{(2+\smallO(1))D^3k^2\vartheta^4}{p} \biggr\} = 1+\smallO(1),
\end{align*}
where the second inequality follows by the Taylor expansion of $x\mapsto \cosh(x)$ and the fact that $\vartheta^2 D = (4+\smallO(1))n\kappa_1\rho^2D/k = \smallO(1)$, and the last equality holds by noting $D^3k^2\vartheta^4/p = (16+\smallO(1)) \kappa_1^2 D^3\rho^4 n^2/p = \smallO(1)$. %This completes the proof.
\end{proof}


